Euler and the Gammafunction

We review Euler's idea on the Gammafunction. We will explain, how Euler obtained them and how Euler's ideas anticipate more modern approaches and theories. Furthermore, some questions asked by Euler are answered.

==> Zusammenfassung.tex <==
\lhead[\thepage]{}
\chead[Deutsche Zusammenfassung der Arbeit]{Euler and the Gamma Function}
\rhead[]{\thepage}
\chapter{Deutsche Zusammenfassung der vorliegenden Arbeit}


%\tableofcontents

\section{Einleitung}

\subsection{Allgemeine Übersicht}

Die nachfolgende Arbeit mit dem Titel "Euler and the Gamma-Function" hat die  Zielsetzung, alle Ergebnisse, welche Leonhard Euler in seiner mathematischen Karriere zur $\Gamma$-Funktion, also der durch das Integral

\begin{equation*}
    \Gamma(x) = \int\limits_{0}^{\infty} e^{-t}t^{x-1}dt \quad \text{für} \quad \operatorname{Re}(x)>0
\end{equation*}
definierten Funktion, zutage gefördert hat, gesammelt darzustellen. Zu diesem Zweck wurden all jene Arbeiten, die entweder direkt der $\Gamma$-Funktion gewidmet sind oder die andere auf die $\Gamma$-Funktion anwendbare Resultate beinhalten, von Eulers lateinischem Original in die deutsche und/oder englische Sprache übersetzt. Dies umfasst insgesamt 13 Arbeiten, die auch, mitsamt ihrem jeweiligen Inhalt, in Sektion 2.3.1 der Hauptarbeit kurz beschrieben werden. Alle Übersetzungen wurden auf der Website des "Euler-Kreis Mainz" zugänglich gemacht. 3 der erwähnten 13 Arbeiten sind aufgrund ihrer hohen Relevanz auch in den Anhang der Hauptarbeit aufgenommen wurden.\\[2mm]

Die Arbeit gliedert sich in 3  Blöcke. \\[2mm]
I. Eine historische Übersicht über die Theorie der $\Gamma$-Funktion von ihrem ersten Auftauchen in einem Brief von Daniel Bernoulli an Goldbach bis zur heutigen Zeit mit besonderem Augenmerk auf Eulers Beiträge. All dies wird in Sektion 2 besprochen. \\[2mm]
II. Eine kurze moderne Einführung in die Theorie der $\Gamma$-Funktion. Dies wird auf zwei Arten erreicht: Zum einen von der Integraldarstellung ausgehend, zum anderen von der Funktionalgleichung, also der Relation

\begin{equation*}
    \Gamma(x+1)=x\Gamma(x)
\end{equation*}
ausgehend. Das erste Vorgehen, Sektion 3 der Arbeit, orientiert sich dabei an Artins Buch, das zweite (Sektion 4) hingegen folgt dem Vorbild von Weierstraß. Auch dabei wird an entsprechender Stelle stets darauf hingewiesen, an welcher Stelle Euler bereits Ideen seiner Nachfolger vorweg genommen hatte, jedoch seine Priorität an selbige abtreten musste.\\[2mm]
III. Eine Erläuterung von Eulers Ansätzen und Beiträgen. Dieser Block unterteilt sich naturgemäß in mehrere Sektionen, von welchen jede einem Zugang Eulers zur $\Gamma$-Funktion gewidmet sind. Dies betrifft die Sektionen 5 bis 9.\\[2mm]

Sektion 10 beinhaltet dann noch eine kurze Zusammenfassung und es wird noch einmal gesondert hervorgehoben, welche Ergebnisse Euler fälschlicherweise zugeschrieben werden sind und für welche ihm Priorität zuschreiben ist.


\subsection{Motivation für die vorliegende Arbeit}

An dieser Stelle wollen wir kurz auf die Beweggründe für die Verfassung dieser Arbeit eingehen, was umso mehr willkommen zu sein scheint, da Arbeiten mit ähnlichem Inhalt bereits von mehreren Autoren verfasst worden sind. Jedoch berücksichtigen letztere, was angesichts Eulers Menge an Abhandlungen auch nachzuvollziehen ist, nicht Eulers gesamten Beitrag. Eine Motivation war es, diese Lücke zu schließen.\\[2mm]
Desweiteren geben die Euler'schen Arbeiten einen wunderbaren Einblick in die Arbeitsweise eines der Giganten der Mathematik. Erfolge sowie Misserfolge bei der Diskussion eines Problems werden in unerreichter Klarheit und in vollem Umfange dargestellt, was sich auch im folgenden, Frobenius zugeschriebenen Zitat widerspiegelt:

\begin{center}
    "He lacked only one thing to make him a perfect genius: He failed to be incomprehensible."
\end{center}
Somit stellen die Euler'schen Arbeiten ein vortreffliches Beispiel f\"ur die "Methodus inveniendi" dar, d.h. die Kunst, wie man eine mathematische Wahrheit \"uberhaupt erst zutage f\"ordert, bevor man zum strengen Beweis derselben  voranschreitet. Die drei im Anhang beigef\"ugten \"Ubersetzungen sind sch\"one Beispiel dessen.\\[2mm]
Nicht zuletzt stellen die Euler'schen Arbeiten gut Dreiviertel der gesamten mathematischen Abhandlungen des 18. Jahrhunderts dar, sodass das ein eingehendes Studium und umfassende Kenntnis derselben f\"ur das  Verst\"andnis der Mathematik und Naturwissenschaften unerl\"asslich sind, sodass wir Zuversichtlich sind, mit der vorliegenden Arbeit, dahingehend einen Beitrag geleistet zu haben.  



\section{Zusammenfassung der einzelnen Sektionen}

Aufgrund der Länge der vorliegenden Arbeit, wollen wir die Gelegenheit nutzen, an dieser Stelle die einzelnen Sektion noch etwas detaillierter zu beschreiben.

\subsection{Historische \"Ubersicht der $\Gamma$-Funktion}

Dieser Abschnitt folgt im Wesentlichen der Darstellung von Davis von der Geburt der $\Gamma$-function bis hin zu den Transzendenzergebnissen der heutigen Zeit. Dass Daniel Bernoulli (und nicht Euler, wie Davis behauptet) der eigentliche Entdecker $\Gamma$-Funktion ist, wird dabei umfassend diskutiert und auch anhand der Originalarbeiten unterlegt (Sektion 2.2). Auf den Euler'schen Beitrag wird in dieser Sektion besonders eingegangen, in Sektion 2.3.2. werden explizit alle Ergebnisse und Formeln genannt, die Euler zur Theorie der $\Gamma$-Funktion beigesteuert hat. Neben der bereits erw\"ahnten Integraldarstellung, sei hier u.A. die Gau\ss{} zugeschriebene Produktdarstellung,

 \begin{equation*}
    x! = \Gamma(x+1) = 1^{1-x} \cdot \dfrac{1^{1-x}2^x}{x+1} \cdot \dfrac{2^{1-x}3^x}{x+2} \cdot \dfrac{3^{1-x}4^x}{x+3} \cdot \text{etc.} = \prod_{k=1}^{\infty} \dfrac{k^{1-x}(k+1)^x}{x+k}.
\end{equation*}
und die Reflexionsformel,

\begin{equation*}
    \dfrac{\pi}{\sin (\pi x)}=\Gamma(x)\Gamma(1-x),
\end{equation*}
genannt. In der vorliegenden Arbeit werden alle Formeln bewiesen, wobei stets der Euler'sche Beweis, gegebenenfalls mit Korrekturen, sowie teilweise auch Beweise, die Euler selbst gef\"uhrt haben k\"onnte, vorgestellt. 

\subsection{Kurze moderne Einf\"uhrung in die Theorie der $\Gamma$-Funktion}

Artins Vorbild folgend, werden von der Integraldarstellung ausgehend (Sektion 3.1.1), die elementaren Eigenschaften der $\Gamma$-Funktion abgeleitet, u.A. die Funktionalgleichung und logarithmische Konvexität sind hier zu nennen (Sektion 3.1.2). Sektion 3.2. enthält dann Klassifikationsätze. Genauer wird in Sektion 3.2.1. Wielandt's Theorem genannt und bewiesen, in Sektion 3.2.2. das Theorem von Bohr-Mollerup, welches zumeist auch als axiomatische Definition der $\Gamma$-Funktion herangezogen wird.



\subsection{L\"osung der Differenzengleichung $F(x+1)=xF(x)$}

Sektion 4.1 folgt dem Weierstra\ss{}'schen Gedanken, die $\Gamma$-Funktion als eindeutige Lösung der Differenzengleichung

\begin{equation*}
    F(x+1)=xF(x)
\end{equation*}
mit der zusätzlichen Bedingung

\begin{equation*}
    \lim_{n \rightarrow \infty} \dfrac{F(x+n)}{(n-1)!n^x}=1.
\end{equation*}
einführt. Die behauptete Eindeutigkeit der Lösung wird demonstriert (Sektion 4.2 und 4.3) und mithilfe des Bohr-Mollerup-Theorems wird die Lösung als $\Gamma$-Funktion erkannt. Als Nebenprodukt ergibt sich in Sektion 4.4 die Weierstra\ss{}'sche Produktdarstellung für die $\Gamma$-Funktion. In Sektion 4.5. wird dann noch diskutiert, dass Euler den Weierstra\ss{}'schen Zugang bezüglich der Einführung der Fakultät bereits vorweg genommen hat.

\subsection{Eulers direkte L\"osung der Gleichung $\Gamma(x+1)=x\Gamma(x)$ - Der Momentenansatz}

Sektion 5.1 beschreibt den Ursprung der Idee - die Euler'sche Methode, homogene Differenzengleichungen mit linearen Koeffizienten zu lösen ist aus dem Verlangen  erwachsen, Kettenbrüche zu summieren. In Sektion 5.2. wird dann mit der Methode die Integraldarstellung der $\Gamma$-Funktion abgeleitet, wohingegen Sektion 5.3. weitere Anwendungsbeispiele enhält. So werden explizite Formeln für die Legendre'schen (Sektion 5.3.1), zu welchen Euler ebenfalls einiges beigetragen hat, wie in Sektion 5.3.2 aufgezeigt wird,  und Hermite'schen Polynome (Sektion 5.3.3) gewonnen. In Sektion 5.3.4 wird die fundamentale Relation 

\begin{equation*}
    B(x,y)=\dfrac{\Gamma(x)\Gamma(y)}{\Gamma(x+y)}
\end{equation*}
aus dem Momentenansatz hergeleitet. Sektion 5.3.6 wendet die Methode auf die hypergeometrische Reihe an.\\
Die Sektionen 5.4 und 5.5. sind dann ganz  modernen mathematischen Theorien, solche Differenzengleichungen aufzulösen, gewidmet. Sektion 5.4 zeigt die Analogie des Euler'schen Vorgehens zur Theorie der Mellin-Transformation auf, wohingegen Sektion 5.5 Differenzengleichungen mithilfe des Schnittzahlenkaklüls löst. Der Euler'sche Ansatz wird analysiert (Sektion 5.5.1), die entscheidenden Begriffe eingeführt (Sektion 5.5.2 und 5.5.3) und die wesentliche Formel abgeleitet (Sektion 5.5.4 bis 5.5.6); die nächsten drei Sektionen (5.5.7 bis 5.5.9) wenden das Hergeleitete auf bereits bekannte Beispiele an, um diesen modernen Zugang zu illustrieren.

\subsection{L\"osung der Differenzengleichung $\log \Gamma(x+1)-\log \Gamma(x) = \log x$ durch Umwandlung in eine Differentialgleichung unendlicher Ordnung}

Nach einer kurzen Übersicht (Sektion 6.1) wird Eulers Ansatz, Differenzengleichungen in Differentialgleichungen zu konvertieren und letztere zu lösen, besprochen (6.2.1) und durch Vergleich mit der eigentlichen Lösung (6.2.2) wird der Fehler in der Euler'schen Argumentation (6.2.3) aufgezeigt. Die folgende Sektion (6.3) ist gänzlich der Behebung des Euler'schen Faupax' gewidmet, wozu in Sektion 6.3.1 alle notwendigen Begriffe und Definitionen aus der Fourieranalysis eingeführt werden. Sektion 6.3.2. gibt dann den Lösungalgorithmus für die allgemeine  Differenzengleichung, was dann in Sektion 6.3.4 auf die speziellere Gleichung

\begin{equation*}
    f(x+1)-f(x)=g(x)
\end{equation*}
angewendet wird. \\
Da die Fourieranalyis nicht bekannt war, wurde in Sektion 6.4 eine formale Lösung gegeben, welche auch Euler selbst vermocht hätte.

\subsection{L\"osung der Gleichung $\log \Gamma(x+1)-\log \Gamma(x) =  \log(x)$ verm\"oge der Euler-Maclaurin'schen Summationsformel}

Nach einer kurzen Übersicht über den Abschnitt (Sektion 7.1) wird die Euler'sche Herleitung der Euler-Maclaurin'schen Summationsformel präsentiert (Sektion 7.2). Sie ergibt sich als spezielle Lösung einer Differenzengleichung, die ebenfalls in eine Differentialgleichung unendlicher Ordnung umgewandelt wird. Die Lösung erfolgt durch einen speziellen Ansatz. Der Vollständigkeit halber wurde in Sektion 7.3. ein kurzer Abriss zur Theorie Differentialgleichungen unendlicher Ordnung gegeben, von Eulers und Bourlets formalen Ansätzen bis hin zur Theorie der Ultradistributionen.
Sektion 7.4. enthält dann noch eine rigorose Herleitung der Euler-Maclaurinschen Summationsformel.

\subsection{Interpolationstheorie und Differenzenkalk\"ul}

In dieser Sektion wird die Euler'sche Lösung des Interpolationsproblem der durch 

\begin{equation*}
    f(x) = \sum_{k=1}^{x} g(k)
\end{equation*}
lediglich für ganzzahlige $x$ definierten Funktion mithilfe des Differenzenkalküls dargestellt. Dabei werden nach der Erläuterung der allgemeinen Idee (Sektion 8.2) zunächst in Sektion 8.3. motivierende Beispiele gegeben (8.3.2. enthält dann die $\Gamma$-Funktion), bevor dann in Sektion 8.4. der Euler'sche Differenzenkalkül eingehend besprochen wird.\\
Sektion 8.5 zeigt dann auf, inwiefern Euler mit seinen Ausführungen bereits die Idee der Weierstra\ss{}'schen Produkte vorweg genommen hat.

\subsection{Beziehung zwischen $\Gamma$ and $B$}

Sektion 9.1 beschreibt den Euler'schen Weg, von der $B$-function zur $\Gamma$-Funktion zu gelangen, wohingegen Sektion 9.2 sich mit der fundamentalen Relation 

\begin{equation*}
    B(x,y)= \dfrac{\Gamma(x)\Gamma(y)}{\Gamma(x+y)}
\end{equation*}
beschäftigt. Neben Eulers heuristischem Argument (Sektion 9.2.1) werden auch die strengen Beweise von Jacobi (Sektion 9.2.2) und Dirichlet (Sektion 9.2.3) besprochen. Sektion 9.3. bespricht dann die Euler'sche Darstellung von der $\Gamma$-Funktion rationaler Werte über $B$-Integrale. Sektion 9.4. enthält den Euler'schen Beweis der Reflektionsformel (Sektion 9.4.2), wobei sich die dafür benötigte Produktdarstellung des Sinus' nach Euler'schem Vorbild in Sektion 9.4.1 findet. Sektion 9.4.3. enthält dann noch einen weiteren elementaren Beweis der Reflektionsformel. Die Ergebnisse von Sektion 9.4. geben dann auch die Gelegenheit, in Sektion 9.5. auf die Gammaklassen (Sektion 9.5.1) und Gammavermutungen (Sektion 9.5.2) zu sprechen zu kommen und eine moderne Anwendung zu geben. Sektion 9.6. handelt dann von der Multiplikationsformel

\begin{equation*}
\Gamma \left(\dfrac{x}{n}\right)\Gamma \left(\dfrac{x+1}{n}\right)\cdots \Gamma \left(\dfrac{x+n-1}{n}\right)= \dfrac{(2\pi)^{\frac{n-1}{2}}}{n^{x-\frac{1}{2}}}\cdot \Gamma(x).
\end{equation*}
und dem Nachweis, dass sich diese bereits in anderer Darstellung in den Euler'schen Abhandlungen findet.

\subsection{Zusammenfassung und Anhang}

Neben einer kurz gehaltenen allgemeinen Zusammenfassung (Sektion 10.1) werden noch einmal gesondert die Euler'schen Ergebnisse hervorgehoben, die nicht mit selbigem assoziiert werden (Sektion 10.1.2), sowie die, welche ihm fälschlicherweise zugesprochen werden (Sektion 10.1.3).\\
Der Anhang, Sektion 11, enthält neben den bereits erwähnten Übersetzungen, noch eine weitere Lösung des Baseler Problems (Sektion 11.1), also der Summation 

\begin{equation*}
    1+\dfrac{1}{2^2}+\dfrac{1}{3^2}+\cdots = \dfrac{\pi^2}{6},
\end{equation*}
welche lediglich auf Eulers Ergebnissen gefußt ist, ihm aber entgangen ist; desweiteren werden Eulers Methode der Partialbruchzerlegung (Sektion 11.2) sowie Eulers Beiträge zur Euler-Mascheroni Konstante $\gamma$ (Sektion 11.3) besprochen.

\section{Danksagung}

An dieser Stelle möchte sich der Autor bei den Betreuern  Professor Tilman Sauer und Professor Duco van Straten für die zahlreichen und hilfreichen Anmerkungen und Diskussionen über die Darstellung des Inhaltes bedanken. Zusätzlich möchte der Autor Professor Vadim Kostrykin bedanken, dessen Anmerkungen für die Erstellung von Sektion 6.3. unerlässlich waren.



